Galaxy counterparts of intervening high-z sub-DLAs/DLAs and MgII absorbers towards gamma-ray bursts

We present the first search for galaxy counterparts of intervening high-z (2<z< 3.6) sub-DLAs and DLAs towards GRBs. Our final sample comprises of five intervening sub-DLAs and DLAs in four GRB fields. To identify candidate galaxy counterparts of the absorbers we use deep optical and near-infrared imaging, and low-, mid- and high-resolution spectroscopy acquired with 6 to 10-m class telescopes, the Hubble and the Spitzer space telescopes. Furthermore, we use the spectroscopic information and spectral-energy-distribution fitting techniques to study them in detail. Our main result is the detection and spectroscopic confirmation of the galaxy counterpart of the intervening DLA at z=3.096 in the field of GRB 070721B (z_GRB=3.6298) as proposed by other authors. We also identify good candidates for the galaxy counterparts of the two strong MgII absorbers at z=0.6915 and 1.4288 towards GRB 050820A (z_GRB=2.615). The properties of the detected DLA galaxy are typical for Lyman-break galaxies (LBGs) at similar redshifts; a young, highly starforming galaxy that shows evidence for a galactic outflow. This supports the hypothesis that a DLA can be the gaseous halo of an LBG. In addition, we report a redshift coincidence of different objects associated with metal lines in the same field, separated by 130-161 kpc. The high detection rate of three correlated structures on a length scale as small as ~150 kpc in two pairs of lines of sight is intriguing. The absorbers in each of these are most likely not part of the same gravitationally bound structure. They more likely represent groups of galaxies.

==> log_data_one_column.tex <==
\begin{sidewaystable*}
\caption{Summary of photometric and spectroscopic data}
\tiny
\begin{tabular}{l c c c c|l c c c c c c c c}

\toprule
\multicolumn{4}{c}{\textbf{Photometry}\tablefootmark{a}}& &\multicolumn{9}{c}{\textbf{Spectroscopy}\tablefootmark{b}}\\[1mm]
\multirow{2}{*}{Instrument}	& \multirow{2}{*}{Filter}	& Exposure			& \multirow{2}{*}{Seeing}	& Photo-		& \multirow{2}{*}{Instrument}	& \multirow{2}{*}{Grating}	& Spectral 		& Resolving	& Exposure 	& Slit 		& Position	& \multirow{2}{*}{Seeing}	& Photo-	\\
				&						& time (s)			&				& metric?		&				&						& range (\AA)		& power		& time (s)	& width		& angle		&				& metric?	\\
\midrule
\multicolumn{10}{l}{\textbf{GRB 050730: $RA=14^{\rm h}08^{\rm m}17\fs11$ $DEC=-03^\circ46'17\farcs70$ (J2000)}}\\
\midrule
VLT/FORS2	& $R$		& $8\times250 + 24\times300$	& 0\farcs6	& yes	& VLT/FORS1			& 600V+GG435	& 4430--7370			& 990			& $5\times1316$		& 1\farcs3			& 22\fdg5		& 0\farcs8	& yes\\
\hst/ACS	& $F775W$	& $6\times1307$			&		&	& \multirow{4}{*}{VLT/FORS2}	& 600B		& 3300--6210			& 780			& $4\times1316$		& 1\farcs3			& -20\fdg0		& 0\farcs9	& yes\\
VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs7	& yes	&				& 300V		& 3400--9500			& 440			& $600+1200$		& 1\farcs0			& 0\fdg0		& 1\farcs5 & no\\
\textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	& \textbf{7200}	&		&	&				& 600B		& 3300--6210			& 780			& $5\times1316$		& 1\farcs3 			& 33\fdg5 		& 1\farcs2	& yes\\
		&		&				&		&	&				& 600B		& 3300--6210 			& 780			& $4\times1316$		& 1\farcs3			& 95\fdg0		& 1\farcs3	& yes\\
		&		&				&		&	& \multirow{2}{*}{VLT/UVES}	& 346 and 580	& 3030--6840\tablefootmark{c}	& \multirow{2}{*}{$\sim40000$}	& \multirow{2}{*}{3000}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{0\fdg0}	& \multirow{1}{*}{1\farcs8}	& \multirow{1}{*}{no}\\
		&		&				&		&	&				& 437 and 860	& 3730--10600\tablefootmark{d}	&				&			&				&				& \multirow{1}{*}{1\farcs1}	& \multirow{1}{*}{yes}\\
		&		&				&		&	& \multirow{3}{*}{VLT/X-shooter\tablefootmark{e}}& UVB	& 3000--5500		& 4000			& $2\times900$		& 1\farcs3			& \multirow{3}{*}{43\fdg7}& \multirow{3}{*}{0\farcs8} & \multirow{3}{*}{yes}\\
		&		&				&		&	&				& VIS		& 5500--10000			& 6700			& $2\times900$		& 1\farcs2			& 			\\
		&		&				&		&	&				& NIR		& 10000--25000			& 4000			& $6\times300$		& 1\farcs2			& 			\\
% \midrule
% \multicolumn{10}{l}{\textbf{GRB 050820A:	$RA=22^{\rm h}29^{\rm m}38\fs114$, $DEC= 19^\circ33'36\farcs61$ (J2000)}}\\
% \midrule
% Keck/LRIS	& $g$		& 2620				& 0\farcs7		& yes		& \multirow{6}{*}{VLT/FORS2}	& 300V		& \multirow{3}{*}{3400--9500}	& \multirow{3}{*}{440}	& $4\times1316$		& 1\farcs3			& -52\fdg0		& 1\farcs2	& yes\\
% \hst/ACS	& $F625W$	& 2238				&		&	&				& 300V		& 				& 			& $8\times1316$		& 1\farcs3			& 34\fdg0		& 1\farcs3	& yes\\
% VLT/FORS2	& $R$		& $4\times500$			& 0\farcs8	& no	&				& 300V		& 				& 			& $4\times1316$		& 1\farcs3			& 83\fdg0		& 0\farcs7	& yes\\
% \hst/ACS	& $F775W$	& 4404				&		&	&				& 1028z+OG590	& \multirow{3}{*}{7730--9480}	& \multirow{3}{*}{2560}	& $2\times1316$		& 1\farcs3			& -52\fdg0		& 0\farcs8	& yes\\
% \hst/ACS	& $F850LP$	& 14280				&		&	&				& 1028z+OG590	& 				&			& $4\times1316$		& 1\farcs3			& 34\fdg0		& 1\farcs2	& yes\\
% Magellan/PANIC	& $H$		& 8460				& 0\farcs6	& 	&				& 1028z+OG590	& 				& 			& $2\times1316$		& 1\farcs3			& 83\fdg0		& 0\farcs7	& yes\\
% VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs7	& yes	& \multirow{2}{*}{VLT/UVES}	& 390 and 564	& 3260--6680\tablefootmark{f}	& \multirow{2}{*}{$\sim40000$}	& \multirow{1}{*}{1800+1815}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{0\fdg0}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{yes}\\
% \textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	&\textbf{3600}	&		&	&				& 437 and 860	& 3730--10600\tablefootmark{d}	& 				& \multirow{1}{*}{2430}		& 				&				& 				& \\
% \midrule
% \multicolumn{10}{l}{\textbf{GRB 050908: $RA=01^{\rm h}21^{\rm m}50\fs73$, $DEC=-12^\circ57'17\farcs30$ (J2000)}}	\\
% \midrule
% VLT/FORS2	& $R$		& $12\times500$			& 0\farcs7	& yes	& Gemini/GMOS-N			& B600+G0305	& 5118--7882			& 844			& $2\times1200$		& 0\farcs75			& 110\fdg0		& \textbf{???} & \textbf{???}\\
% VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs6	& yes	& \multirow{2}{*}{VLT/FORS1}	& 300V		& 3400--9500			& 440			& $3\times1200$		& 1\farcs0			& 0\fdg0		& 0\farcs6 & yes\\
% \textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	&\textbf{7200}		&	 	& 	&				& 600B		& 3300--6210			& 780			& $6\times1345$		& 1\farcs3			& 53\fdg8		& 1\farcs2 & yes\\
% \midrule
% \multicolumn{10}{l}{\textbf{GRB 070721B: $RA=02^{\rm h}12^{\rm m}32\fs95$, $DEC=-02^\circ11'40\farcs80$ (J2000)}}\\
% \midrule
% VLT/FORS2	& $R$		& $24\times235$			& 0\farcs5	& no	& VLT/FORS1			& 300V		& 3400--9500			& 440			& $5\times2735$		& 1\farcs3			& -118\fdg5		& 1\farcs2	& yes\\
% \hst/ACS	& $F775W$	& $6\times1307$			& 		&	& VLT/FORS2			& 300V		& 3400--9500			& 440			& $4\times1800$		& 1\farcs0			& -118\fdg3		& 1\farcs2 & yes\\
% Magellan/PANIC	& $H$		& 10320				& 0\farcs5	&	\\
% VLT/ISAAC	& $K_s$		& $32\times60$			& 1\farcs0	& yes	\\
\bottomrule
\end{tabular}
  \tablefoot{Co-ordinates were taken from \citet{Malesani2012a}.
	\textbf{Photometry}: Observing conditions of Keck and Magellan data are quoted from \citet{Chen2009a}.
	Column "Photometric?" states if observing conditions were photometric.
	\textbf{Spectroscopy}:
	Observing conditions of the afterglow spectroscopy campaigns, and the VLT/UVES data of GRB
	050730 are taken from \citet{Fynbo2009a}, \citet{Ledoux2009a}, and
	\citet{Vergani2009a}.
	\textbf{The} VLT/UVES and VLT/X-shooter spectrographs consist of two and three arms, respectively, displayed
	in the column "Grating". Observations in the different arms are carried out simultaneously.
	Resolving power of VLT/FORS1+2 grisms are given for a slit width of $1''$.
	The stated resolving power of the X-shooter NIR spectrum was decreased during the data reduction
	to increase S/N. The effective resolving power of the X-shooter NIR arm is around ten times
	lower.
	\tablefoottext{a} Date of observations.
	GRB 050730:	VLT/FORS2 - 2006/03/04 - 05/25, \hst/ACS - 2010/06/10, VLT/ISAAC - 2006/03/20, \textbf{\spitzer/IRAC: 2008/03/11};
% 	GRB 050820A: 	Keck/LRIS - July 2006, \hst/ACS - $F625W$, $F775W$, $F850LP$: 2005/09/26 and 2006/06/05-11, Magellan/PANIC: August 2007, VLT/FORS2 - 2006/05/24, VLT/ISAAC - 2006/05/20, \textbf{\spitzer: 2007/12/23};
% 	GRB 050908:	VLT/FORS2 - 2007/07/21-08/14, VLT/ISAAC - 2007/07/11, \textbf{\spitzer/IRAC: 2008/08/18};
% 	GRB 070721B:	VLT/FORS2 - 2007/10/04-11/13, \hst/ACS - 2010/11/13, Magellan/PANIC - August 2007, VLT/ISAAC - 2007/09/22.
	\tablefoottext{b} Date of observations.
	GRB 050730:	VLT/FORS1 600V+GG435 - 2007/02/23-24, VLT/FORS2 600B - $\rm{PA}=20\fdg0$: 2006/06/22, $\rm{PA}=0\fdg0$: 2005/07/31, $\rm{PA}=33\fdg5$: 2006/04/28-05/28, $\rm{PA}=95\fdg0$: 2006/05/28, VLT/UVES: 2005/07/31, VLT/X-shooter: 2010/04/18;
% 	GRB 050820A: 	VLT/FORS2 300V - $\rm{PA}=-52\fdg0$: 2006/07/22-08/16, $\rm{PA}=34\fdg0$: 2006/08/31-09/22, $\rm{PA}=83\fdg0$: 2006/08/17-09/15, 1028z - $\rm{PA}=-52\fdg0$: 2006/08/16, $\rm{PA}=34\fdg0$: 2006/09/17-22, $\rm{PA}=83\fdg0$: 2006/08/17, VLT/UVES: 2005/08/20;
% 	GRB 050908:	Gemini/GMOS-N - 2005/09/08, VLT/FORS1 - 300V: 2005/09/08, 600B: 2007/08/16-09/06; 
% 	GRB 070721B:	VLT/FORS1 - 2007/11/16-12/04, VLT/FORS2 - 2007/07/22.
	\tablefoottext{c} Spectral range of the blue and red arms are 3030--3880 \AA~and 4760--6840 \AA, respectively.
	\tablefoottext{d} Spectral range of the blue and red arms are 3730--4990 \AA~and 6600--10600 \AA, respectively.
	\tablefoottext{e} The target of the X-shooter observation was QSO J1408-0346.
% 	\tablefoottext{f} Spectral range of the blue and red arms are 3260--4450 \AA~and 4580--6680 \AA, respectively.
} 
\label{tab:log_photometry}
\end{sidewaystable*}

\begin{sidewaystable*}
% \caption{Summary of photometric and spectroscopic data}
\tiny
\begin{tabular}{l c c c c|l c c c c c c c c}

\toprule
\multicolumn{4}{c}{\textbf{Photometry}\tablefootmark{a}}& &\multicolumn{9}{c}{\textbf{Spectroscopy}\tablefootmark{b}}\\[1mm]
\multirow{2}{*}{Instrument}	& \multirow{2}{*}{Filter}	& Exposure			& \multirow{2}{*}{Seeing}	& Photo-		& \multirow{2}{*}{Instrument}	& \multirow{2}{*}{Grating}	& Spectral 		& Resolving	& Exposure 	& Slit 		& Position	& \multirow{2}{*}{Seeing}	& Photo-	\\
				&						& time (s)			&				& metric?		&				&						& range (\AA)		& power		& time (s)	& width		& angle		&				& metric?	\\
% \midrule
% \multicolumn{10}{l}{\textbf{GRB 050730: $RA=14^{\rm h}08^{\rm m}17\fs11$ $DEC=-03^\circ46'17\farcs70$ (J2000)}}\\
% \midrule
% VLT/FORS2	& $R$		& $8\times250 + 24\times300$	& 0\farcs6	& yes	& VLT/FORS1			& 600V+GG435	& 4430--7370			& 990			& $5\times1316$		& 1\farcs3			& 22\fdg5		& 0\farcs8	& yes\\
% \hst/ACS	& $F775W$	& $6\times1307$			&		&	& \multirow{4}{*}{VLT/FORS2}	& 600B		& 3300--6210			& 780			& $4\times1316$		& 1\farcs3			& -20\fdg0		& 0\farcs9	& yes\\
% VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs7	& yes	&				& 300V		& 3400--9500			& 440			& $600+1200$		& 1\farcs0			& 0\fdg0		& 1\farcs5 & no\\
% \textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	& \textbf{7200}	&		&	&				& 600B		& 3300--6210			& 780			& $5\times1316$		& 1\farcs3 			& 33\fdg5 		& 1\farcs2	& yes\\
% 		&		&				&		&	&				& 600B		& 3300--6210 			& 780			& $4\times1316$		& 1\farcs3			& 95\fdg0		& 1\farcs3	& yes\\
% 		&		&				&		&	& \multirow{2}{*}{VLT/UVES}	& 346 and 580	& 3030--6840\tablefootmark{c}	& \multirow{2}{*}{$\sim40000$}	& \multirow{2}{*}{3000}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{0\fdg0}	& \multirow{1}{*}{1\farcs8}	& \multirow{1}{*}{no}\\
% 		&		&				&		&	&				& 437 and 860	& 3730--10600\tablefootmark{d}	&				&			&				&				& \multirow{1}{*}{1\farcs1}	& \multirow{1}{*}{yes}\\
% 		&		&				&		&	& \multirow{3}{*}{VLT/X-shooter\tablefootmark{e}}& UVB	& 3000--5500		& 4000			& $2\times900$		& 1\farcs3			& \multirow{3}{*}{43\fdg7}& \multirow{3}{*}{0\farcs8} & \multirow{3}{*}{yes}\\
% 		&		&				&		&	&				& VIS		& 5500--10000			& 6700			& $2\times900$		& 1\farcs2			& 			\\
% 		&		&				&		&	&				& NIR		& 10000--25000			& 4000			& $6\times300$		& 1\farcs2			& 			\\
\midrule
\multicolumn{10}{l}{\textbf{GRB 050820A:	$RA=22^{\rm h}29^{\rm m}38\fs114$, $DEC= 19^\circ33'36\farcs61$ (J2000)}}\\
\midrule
Keck/LRIS	& $g$		& 2620				& 0\farcs7		& yes		& \multirow{6}{*}{VLT/FORS2}	& 300V		& \multirow{3}{*}{3400--9500}	& \multirow{3}{*}{440}	& $4\times1316$		& 1\farcs3			& -52\fdg0		& 1\farcs2	& yes\\
\hst/ACS	& $F625W$	& 2238				&		&	&				& 300V		& 				& 			& $8\times1316$		& 1\farcs3			& 34\fdg0		& 1\farcs3	& yes\\
VLT/FORS2	& $R$		& $4\times500$			& 0\farcs8	& no	&				& 300V		& 				& 			& $4\times1316$		& 1\farcs3			& 83\fdg0		& 0\farcs7	& yes\\
\hst/ACS	& $F775W$	& 4404				&		&	&				& 1028z+OG590	& \multirow{3}{*}{7730--9480}	& \multirow{3}{*}{2560}	& $2\times1316$		& 1\farcs3			& -52\fdg0		& 0\farcs8	& yes\\
\hst/ACS	& $F850LP$	& 14280				&		&	&				& 1028z+OG590	& 				&			& $4\times1316$		& 1\farcs3			& 34\fdg0		& 1\farcs2	& yes\\
Magellan/PANIC	& $H$		& 8460				& 0\farcs6	& 	&				& 1028z+OG590	& 				& 			& $2\times1316$		& 1\farcs3			& 83\fdg0		& 0\farcs7	& yes\\
VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs7	& yes	& \multirow{2}{*}{VLT/UVES}	& 390 and 564	& 3260--6680\tablefootmark{f}	& \multirow{2}{*}{$\sim40000$}	& \multirow{1}{*}{1800+1815}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{0\fdg0}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{yes}\\
\textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	&\textbf{3600}	&		&	&				& 437 and 860	& 3730--10600\tablefootmark{d}	& 				& \multirow{1}{*}{2430}		& 				&				& 				& \\
% \midrule
% \multicolumn{10}{l}{\textbf{GRB 050908: $RA=01^{\rm h}21^{\rm m}50\fs73$, $DEC=-12^\circ57'17\farcs30$ (J2000)}}	\\
% \midrule
% VLT/FORS2	& $R$		& $12\times500$			& 0\farcs7	& yes	& Gemini/GMOS-N			& B600+G0305	& 5118--7882			& 844			& $2\times1200$		& 0\farcs75			& 110\fdg0		& \textbf{???} & \textbf{???}\\
% VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs6	& yes	& \multirow{2}{*}{VLT/FORS1}	& 300V		& 3400--9500			& 440			& $3\times1200$		& 1\farcs0			& 0\fdg0		& 0\farcs6 & yes\\
% \textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	&\textbf{7200}		&	 	& 	&				& 600B		& 3300--6210			& 780			& $6\times1345$		& 1\farcs3			& 53\fdg8		& 1\farcs2 & yes\\
% \midrule
% \multicolumn{10}{l}{\textbf{GRB 070721B: $RA=02^{\rm h}12^{\rm m}32\fs95$, $DEC=-02^\circ11'40\farcs80$ (J2000)}}\\
% \midrule
% VLT/FORS2	& $R$		& $24\times235$			& 0\farcs5	& no	& VLT/FORS1			& 300V		& 3400--9500			& 440			& $5\times2735$		& 1\farcs3			& -118\fdg5		& 1\farcs2	& yes\\
% \hst/ACS	& $F775W$	& $6\times1307$			& 		&	& VLT/FORS2			& 300V		& 3400--9500			& 440			& $4\times1800$		& 1\farcs0			& -118\fdg3		& 1\farcs2 & yes\\
% Magellan/PANIC	& $H$		& 10320				& 0\farcs5	&	\\
% VLT/ISAAC	& $K_s$		& $32\times60$			& 1\farcs0	& yes	\\
\bottomrule
\end{tabular}
  \tablefoot{Co-ordinates were taken from \citet{Malesani2012a}.
	\textbf{Photometry}: Observing conditions of Keck and Magellan data are quoted from \citet{Chen2009a}.
	Column "Photometric?" states if observing conditions were photometric.
	\textbf{Spectroscopy}:
	Observing conditions of the afterglow spectroscopy campaigns, and the VLT/UVES data of GRB
	GRB 050820A are taken from \citet{Fynbo2009a}, \citet{Ledoux2009a}, and \citet{Vergani2009a}.
	\textbf{The} VLT/UVES spectrograph consists of two and three arms, respectively, displayed
	in the column "Grating". Observations in the different arms are carried out simultaneously.
	Resolving power of VLT/FORS1+2 grisms are given for a slit width of $1''$.
	The stated resolving power of the X-shooter NIR spectrum was decreased during the data reduction
	to increase S/N. The effective resolving power of the X-shooter NIR arm is around ten times
	lower.
	\tablefoottext{a} Date of observations.
% 	GRB 050730:	VLT/FORS2 - 2006/03/04 - 05/25, \hst/ACS - 2010/06/10, VLT/ISAAC - 2006/03/20, \textbf{\spitzer/IRAC: 2008/03/11};
	GRB 050820A: 	Keck/LRIS - July 2006, \hst/ACS - $F625W$, $F775W$, $F850LP$: 2005/09/26 and 2006/06/05-11, Magellan/PANIC: August 2007, VLT/FORS2 - 2006/05/24, VLT/ISAAC - 2006/05/20, \textbf{\spitzer: 2007/12/23};
% 	GRB 050908:	VLT/FORS2 - 2007/07/21-08/14, VLT/ISAAC - 2007/07/11, \textbf{\spitzer/IRAC: 2008/08/18};
% 	GRB 070721B:	VLT/FORS2 - 2007/10/04-11/13, \hst/ACS - 2010/11/13, Magellan/PANIC - August 2007, VLT/ISAAC - 2007/09/22.
	\tablefoottext{b} Date of observations.
% 	GRB 050730:	VLT/FORS1 600V+GG435 - 2007/02/23-24, VLT/FORS2 600B - $\rm{PA}=20\fdg0$: 2006/06/22, $\rm{PA}=0\fdg0$: 2005/07/31, $\rm{PA}=33\fdg5$: 2006/04/28-05/28, $\rm{PA}=95\fdg0$: 2006/05/28, VLT/UVES: 2005/07/31, VLT/X-shooter: 2010/04/18;
	GRB 050820A: 	VLT/FORS2 300V - $\rm{PA}=-52\fdg0$: 2006/07/22-08/16, $\rm{PA}=34\fdg0$: 2006/08/31-09/22, $\rm{PA}=83\fdg0$: 2006/08/17-09/15, 1028z - $\rm{PA}=-52\fdg0$: 2006/08/16, $\rm{PA}=34\fdg0$: 2006/09/17-22, $\rm{PA}=83\fdg0$: 2006/08/17, VLT/UVES: 2005/08/20;
% 	GRB 050908:	Gemini/GMOS-N - 2005/09/08, VLT/FORS1 - 300V: 2005/09/08, 600B: 2007/08/16-09/06; 
% 	GRB 070721B:	VLT/FORS1 - 2007/11/16-12/04, VLT/FORS2 - 2007/07/22.
% 	\tablefoottext{c} Spectral range of the blue and red arms are 3030--3880 \AA~and 4760--6840 \AA, respectively.
	\tablefoottext{d} Spectral range of the blue and red arms are 3730--4990 \AA~and 6600--10600 \AA, respectively.
% 	\tablefoottext{e} The target of the X-shooter observation was QSO J1408-0346.
	\tablefoottext{f} Spectral range of the blue and red arms are 3260--4450 \AA~and 4580--6680 \AA, respectively.
} 
% \label{tab:log_photometry}
\hfill\center{Tab. \ref{tab:log_photometry} --- continued}
\end{sidewaystable*}

\begin{sidewaystable*}
% \caption{Summary of photometric and spectroscopic data}
\tiny
\begin{tabular}{l c c c c|l c c c c c c c c}

\toprule
\multicolumn{4}{c}{\textbf{Photometry}\tablefootmark{a}}& &\multicolumn{9}{c}{\textbf{Spectroscopy}\tablefootmark{b}}\\[1mm]
\multirow{2}{*}{Instrument}	& \multirow{2}{*}{Filter}	& Exposure			& \multirow{2}{*}{Seeing}	& Photo-		& \multirow{2}{*}{Instrument}	& \multirow{2}{*}{Grating}	& Spectral 		& Resolving	& Exposure 	& Slit 		& Position	& \multirow{2}{*}{Seeing}	& Photo-	\\
				&						& time (s)			&				& metric?		&				&						& range (\AA)		& power		& time (s)	& width		& angle		&				& metric?	\\
% \midrule
% \multicolumn{10}{l}{\textbf{GRB 050730: $RA=14^{\rm h}08^{\rm m}17\fs11$ $DEC=-03^\circ46'17\farcs70$ (J2000)}}\\
% \midrule
% VLT/FORS2	& $R$		& $8\times250 + 24\times300$	& 0\farcs6	& yes	& VLT/FORS1			& 600V+GG435	& 4430--7370			& 990			& $5\times1316$		& 1\farcs3			& 22\fdg5		& 0\farcs8	& yes\\
% \hst/ACS	& $F775W$	& $6\times1307$			&		&	& \multirow{4}{*}{VLT/FORS2}	& 600B		& 3300--6210			& 780			& $4\times1316$		& 1\farcs3			& -20\fdg0		& 0\farcs9	& yes\\
% VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs7	& yes	&				& 300V		& 3400--9500			& 440			& $600+1200$		& 1\farcs0			& 0\fdg0		& 1\farcs5 & no\\
% \textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	& \textbf{7200}	&		&	&				& 600B		& 3300--6210			& 780			& $5\times1316$		& 1\farcs3 			& 33\fdg5 		& 1\farcs2	& yes\\
% 		&		&				&		&	&				& 600B		& 3300--6210 			& 780			& $4\times1316$		& 1\farcs3			& 95\fdg0		& 1\farcs3	& yes\\
% 		&		&				&		&	& \multirow{2}{*}{VLT/UVES}	& 346 and 580	& 3030--6840\tablefootmark{c}	& \multirow{2}{*}{$\sim40000$}	& \multirow{2}{*}{3000}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{0\fdg0}	& \multirow{1}{*}{1\farcs8}	& \multirow{1}{*}{no}\\
% 		&		&				&		&	&				& 437 and 860	& 3730--10600\tablefootmark{d}	&				&			&				&				& \multirow{1}{*}{1\farcs1}	& \multirow{1}{*}{yes}\\
% 		&		&				&		&	& \multirow{3}{*}{VLT/X-shooter\tablefootmark{e}}& UVB	& 3000--5500		& 4000			& $2\times900$		& 1\farcs3			& \multirow{3}{*}{43\fdg7}& \multirow{3}{*}{0\farcs8} & \multirow{3}{*}{yes}\\
% 		&		&				&		&	&				& VIS		& 5500--10000			& 6700			& $2\times900$		& 1\farcs2			& 			\\
% 		&		&				&		&	&				& NIR		& 10000--25000			& 4000			& $6\times300$		& 1\farcs2			& 			\\
% \midrule
% \multicolumn{10}{l}{\textbf{GRB 050820A:	$RA=22^{\rm h}29^{\rm m}38\fs114$, $DEC= 19^\circ33'36\farcs61$ (J2000)}}\\
% \midrule
% Keck/LRIS	& $g$		& 2620				& 0\farcs7		& yes		& \multirow{6}{*}{VLT/FORS2}	& 300V		& \multirow{3}{*}{3400--9500}	& \multirow{3}{*}{440}	& $4\times1316$		& 1\farcs3			& -52\fdg0		& 1\farcs2	& yes\\
% \hst/ACS	& $F625W$	& 2238				&		&	&				& 300V		& 				& 			& $8\times1316$		& 1\farcs3			& 34\fdg0		& 1\farcs3	& yes\\
% VLT/FORS2	& $R$		& $4\times500$			& 0\farcs8	& no	&				& 300V		& 				& 			& $4\times1316$		& 1\farcs3			& 83\fdg0		& 0\farcs7	& yes\\
% \hst/ACS	& $F775W$	& 4404				&		&	&				& 1028z+OG590	& \multirow{3}{*}{7730--9480}	& \multirow{3}{*}{2560}	& $2\times1316$		& 1\farcs3			& -52\fdg0		& 0\farcs8	& yes\\
% \hst/ACS	& $F850LP$	& 14280				&		&	&				& 1028z+OG590	& 				&			& $4\times1316$		& 1\farcs3			& 34\fdg0		& 1\farcs2	& yes\\
% Magellan/PANIC	& $H$		& 8460				& 0\farcs6	& 	&				& 1028z+OG590	& 				& 			& $2\times1316$		& 1\farcs3			& 83\fdg0		& 0\farcs7	& yes\\
% VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs7	& yes	& \multirow{2}{*}{VLT/UVES}	& 390 and 564	& 3260--6680\tablefootmark{f}	& \multirow{2}{*}{$\sim40000$}	& \multirow{1}{*}{1800+1815}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{0\fdg0}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{yes}\\
% \textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	&\textbf{3600}	&		&	&				& 437 and 860	& 3730--10600\tablefootmark{d}	& 				& \multirow{1}{*}{2430}		& 				&				& 				& \\
% \midrule
\multicolumn{10}{l}{\textbf{GRB 050908: $RA=01^{\rm h}21^{\rm m}50\fs73$, $DEC=-12^\circ57'17\farcs30$ (J2000)}}	\\
\midrule
VLT/FORS2	& $R$		& $12\times500$			& 0\farcs7	& yes	& Gemini/GMOS-N			& B600+G0305	& 5118--7882			& 844			& $2\times1200$		& 0\farcs75			& 110\fdg0		& 		&\\
VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs6	& yes	& \multirow{2}{*}{VLT/FORS1}	& 300V		& 3400--9500			& 440			& $3\times1200$		& 1\farcs0			& 0\fdg0		& 0\farcs6 & yes\\
\textbf{\spitzer/IRAC}	& \textbf{$3.6\,\&\,5.8\,\mu\rm m$}	&\textbf{7200}		&	 	& 	&				& 600B		& 3300--6210			& 780			& $6\times1345$		& 1\farcs3			& 53\fdg8		& 1\farcs2 & yes\\
\midrule
\multicolumn{10}{l}{\textbf{GRB 070721B: $RA=02^{\rm h}12^{\rm m}32\fs95$, $DEC=-02^\circ11'40\farcs80$ (J2000)}}\\
\midrule
VLT/FORS2	& $R$		& $24\times235$			& 0\farcs5	& no	& VLT/FORS1			& 300V		& 3400--9500			& 440			& $5\times2735$		& 1\farcs3			& -118\fdg5		& 1\farcs2	& yes\\
\hst/ACS	& $F775W$	& $6\times1307$			& 		&	& VLT/FORS2			& 300V		& 3400--9500			& 440			& $4\times1800$		& 1\farcs0			& -118\fdg3		& 1\farcs2 & yes\\
Magellan/PANIC	& $H$		& 10320				& 0\farcs5	&	\\
VLT/ISAAC	& $K_s$		& $32\times60$			& 1\farcs0	& yes	\\
\bottomrule
\end{tabular}
  \tablefoot{Co-ordinates were taken from \citet{Malesani2012a}.
	\textbf{Photometry}: Observing conditions of Keck and Magellan data are quoted from \citet{Chen2009a}.
	Column "Photometric?" states if observing conditions were photometric.
% 	\textbf{Spectroscopy}:
	Observing conditions of the afterglow spectroscopy campaigns are taken from \citet{Fynbo2009a}.
% 	\textbf{The} VLT/UVES and VLT/X-shooter spectrographs consist of two and three arms, respectively, displayed
% 	in the column "Grating". Observations in the different arms are carried out simultaneously.
	Resolving power of VLT/FORS1+2 and Gemini grisms are given for a slit width of $1''$.
	The stated resolving power of the X-shooter NIR spectrum was decreased during the data reduction
	to increase S/N. The effective resolving power of the X-shooter NIR arm is around ten times
	lower.
	\tablefoottext{a} Date of observations.
% 	GRB 050730:	VLT/FORS2 - 2006/03/04 - 05/25, \hst/ACS - 2010/06/10, VLT/ISAAC - 2006/03/20, \textbf{\spitzer/IRAC: 2008/03/11};
% 	GRB 050820A: 	Keck/LRIS - July 2006, \hst/ACS - $F625W$, $F775W$, $F850LP$: 2005/09/26 and 2006/06/05-11, Magellan/PANIC: August 2007, VLT/FORS2 - 2006/05/24, VLT/ISAAC - 2006/05/20, \textbf{\spitzer: 2007/12/23};
	GRB 050908:	VLT/FORS2 - 2007/07/21-08/14, VLT/ISAAC - 2007/07/11, \textbf{\spitzer/IRAC: 2008/08/18};
	GRB 070721B:	VLT/FORS2 - 2007/10/04-11/13, \hst/ACS - 2010/11/13, Magellan/PANIC - August 2007, VLT/ISAAC - 2007/09/22.
	\tablefoottext{b} Date of observations.
% 	GRB 050730:	VLT/FORS1 600V+GG435 - 2007/02/23-24, VLT/FORS2 600B - $\rm{PA}=20\fdg0$: 2006/06/22, $\rm{PA}=0\fdg0$: 2005/07/31, $\rm{PA}=33\fdg5$: 2006/04/28-05/28, $\rm{PA}=95\fdg0$: 2006/05/28, VLT/UVES: 2005/07/31, VLT/X-shooter: 2010/04/18;
% 	GRB 050820A: 	VLT/FORS2 300V - $\rm{PA}=-52\fdg0$: 2006/07/22-08/16, $\rm{PA}=34\fdg0$: 2006/08/31-09/22, $\rm{PA}=83\fdg0$: 2006/08/17-09/15, 1028z - $\rm{PA}=-52\fdg0$: 2006/08/16, $\rm{PA}=34\fdg0$: 2006/09/17-22, $\rm{PA}=83\fdg0$: 2006/08/17, VLT/UVES: 2005/08/20;
	GRB 050908:	Gemini/GMOS-N - 2005/09/08, VLT/FORS1 - 300V: 2005/09/08, 600B: 2007/08/16-09/06; 
	GRB 070721B:	VLT/FORS1 - 2007/11/16-12/04, VLT/FORS2 - 2007/07/22.
% 	\tablefoottext{c} Spectral range of the blue and red arms are 3030--3880 \AA~and 4760--6840 \AA, respectively.
% 	\tablefoottext{d} Spectral range of the blue and red arms are 3730--4990 \AA~and 6600--10600 \AA, respectively.
% 	\tablefoottext{e} The target of the X-shooter observation was QSO J1408-0346.
% 	\tablefoottext{f} Spectral range of the blue and red arms are 3260--4450 \AA~and 4580--6680 \AA, respectively.
} 
% \label{tab:log_photometry}
\hfill\center{Tab. \ref{tab:log_photometry} --- continued}
\end{sidewaystable*}

==> log_photometry.tex <==
%\begin{sidewaystable*}
\begin{landscape}
\begin{table*}
\caption{Summary of photometric and spectroscopic data}
\centering
\tiny
\begin{tabular}{l c c c c|l c c c c c c c c}
\toprule
\multicolumn{4}{c}{\textbf{Photometry}}& &\multicolumn{7}{c}{\textbf{Spectroscopy}}\\[1mm]
\multirow{2}{*}{Instrument}	& \multirow{2}{*}{Filter}	& Exposure			& \multirow{2}{*}{Seeing}	& Photo-		& \multirow{2}{*}{Instrument}	& \multirow{2}{*}{Grating}	& Spectral 		& Resolving	& Exposure 	& Slit 		& Position	& \multirow{2}{*}{Seeing}	& Photo-	\\
							&							& time (s)			&							& metric?		&								&							& range (\AA)	& power		& time (s)	& width		& angle		&							& metric?	\\
\midrule
\multicolumn{10}{l}{\textbf{GRB 050730: $RA=14^{\rm h}08^{\rm m}17\fs11$ $DEC=-03^\circ46'17\farcs70$ (J2000)}}\\
\midrule
VLT/FORS2	& $R$		& $8\times250 + 24\times300$	& 0\farcs6	& no	& VLT/FORS1			& 600V+GG435	& 4430--7370			& 990			& $5\times1316$		& 1\farcs3			& 22\fdg5		& 0\farcs8	& yes\\
\hst/ACS	& $F775W$	& $6\times1307$			&		&	& \multirow{4}{*}{VLT/FORS2}	& 600B		& 3300--6210			& 780			& $4\times1316$		& 1\farcs3			& -20\fdg0		& 0\farcs9	& yes\\
VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs7	& yes	&				& 300V		& 3400--9500			& 440			& $600+1200$		& 1\farcs0			& 0\fdg0		\\
		&		&				&		&	&				& 600B		& 3300--6210			& 780			& $5\times1316$		& 1\farcs3 			& 33\fdg5 		& 1\farcs2	& yes\\
		&		&				&		&	&				& 600B		& 3300--6210 			& 780			& $4\times1316$		& 1\farcs3			& 95\fdg0		& 1\farcs3	& yes\\
		&		&				&		&	& \multirow{2}{*}{VLT/UVES\tablefootmark{a}}& 346& 3030--3880 			& $\sim47000$		& \multirow{2}{*}{3000}	& \multirow{2}{*}{1\farcs0}	& \multirow{2}{*}{0\fdg0}\\
		&		&				&		&	& 				&580		&4760--6840			& $\sim45000$		& 			&				& 			\\
		&		&				&		&	& \multirow{3}{*}{VLT/X-shooter\tablefootmark{b}}& UVB	& 3000--5500		& 4000			& $2\times900$		& 1\farcs3			& \multirow{3}{*}{43\fdg7}& \multirow{3}{*}{0.8} & \multirow{3}{*}{yes}\\
		&		&				&		&	&				& VIS		& 5500--10000			& 6700			& $2\times900$		& 1\farcs2			& 			\\
		&		&				&		&	&				& NIR		& 10000--25000			& 4000			& $6\times300$		& 1\farcs2			& 			\\
\midrule
\multicolumn{10}{l}{\textbf{GRB 050820A:	$RA=22^{\rm h}29^{\rm m}38\fs11$, $DEC= 19^\circ33'36\farcs61$ (J2000)}}\\
\midrule
Keck/LRIS	& $g$		& 2620				&		&	& \multirow{6}{*}{VLT/FORS2}	& 300V		& \multirow{3}{*}{3400--9500}	& \multirow{3}{*}{440}	& $4\times1316$		& 1\farcs3			& -52\fdg0		& 1\farcs2	& yes\\
\hst/ACS	& $F625W$	& 2238				&		&	&				& 300V		& 				& 			& $8\times1316$		& 1\farcs3			& 34\fdg0		& 1\farcs3	& yes\\
VLT/FORS2	& $R$		& $4\times500$			& 0\farcs8	& no	&				& 300V		& 				& 			& $4\times1316$		& 1\farcs3			& 83\fdg0		& 0\farcs7	& yes\\
\hst/ACS	& $F775W$	& 4404				&		&	&				& 1028z+OG590	& \multirow{3}{*}{7730--9480}	& \multirow{3}{*}{2560}	& $2\times1316$		& 1\farcs3			& -52\fdg0		& 0\farcs8	& yes\\
\hst/ACS	& $F850LP$	& 14280				&		&	&				& 1028z+OG590	& 				&			& $4\times1316$		& 1\farcs3			& 34\fdg0		& 1\farcs2	& yes\\
Magellan/PANIC	& $H$		& 8460				& 		&	&				& 1028z+OG590	& 				& 			& $2\times1316$		& 1\farcs3			& 83\fdg0		& 0\farcs7	& yes\\
VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs7	& yes	\\
\midrule
\multicolumn{10}{l}{\textbf{GRB 050908: $RA=01^{\rm h}21^{\rm m}50\fs73$, $DEC=-12^\circ57'17\farcs30$ (J2000)}}	\\
\midrule
  VLT/FORS2	& $R$		& $12\times500$			& 0\farcs7	& no	& \multirow{2}{*}{VLT/FORS1}	& 300V		& 3400--9500			& 440			& $3\times1200$		& 1\farcs0			& 0\fdg0		\\
VLT/ISAAC	& $K_s$		& $32\times60$			& 0\farcs6	& yes	& 				& 600B		& 3300--6210			& 780			& $6\times1345$		& 1\farcs3			& 53\fdg8		& 1\farcs2	& yes\\
		&		&				&		&	& Gemini/GMOS-N			& B600+G0305	& 5118--7882			& 844			& $2\times1200$		& 0\farcs75			& 110\fdg0		\\
\midrule
\multicolumn{10}{l}{\textbf{GRB 070721B: $RA=02^{\rm h}12^{\rm m}32\fs95$, $DEC=-02^\circ11'40\farcs80$ (J2000)}}\\
\midrule
VLT/FORS2	& $R$		& $24\times235$			& 0\farcs5	& no	& VLT/FORS1			& 300V		& 3400--9500			& 440			& $5\times2735$		& 1\farcs3			& -118\fdg5		& 1\farcs2	& yes\\
\hst/ACS	& $F775W$	& $6\times1307$			& 		&	& VLT/FORS2			& 300V		& 3400--9500			& 440			& $4\times1800$		& 1\farcs0			& -118\fdg3		\\
Magellan/PANIC	& $H$		& 10320				&		&	\\
VLT/ISAAC	& $K_s$		& $32\times60$			& 1\farcs0	& yes	\\
\bottomrule
\end{tabular}
  \tablefoot{Co-ordinates were taken from Malesani et al., in prep.
	\textbf{Photometry}: We only present the observing conditions for VLT data. Observing
	conditions of Keck and Magellan data and of the \hst~observation of GRB 050820A are presented in \citet{Chen2009a}. Column "Photometric?"
	states if observing conditions were photometric.
	\textbf{Spectroscopy}:
	\textbf{The} VLT/UVES and VLT/X-shooter spectrographs consist of two and three arms, respectively, displayed
	in the column "Grating". Observations in the different arms are carried out simultaneously.
	Resolving power of VLT/FORS1/2 and Gemini gratings are given for a slit width of $1''$.
	Resolving power of the X-shooter NIR spectrum was reduced in order to increase S/N, leading to
	around ten times lower resolving power. Position angle is abbreviated by PA. \tablefoottext{a}
	The target of the X-shooter observation was QSO J1408-0346 in the field of GRB 050730.
} 
\label{tab:log_photometry}
\end{table*}
\end{landscape}
%\end{sidewaystable*}


==> sed_figures.tex <==
\begin{figure}
 \centering
 \includegraphics[bb= 3 8 685 586, clip, width=0.5\textwidth, angle=0]{Figures/GRB050820A_B12.eps}
 \caption{
 	Smoothed Spectrum (top) and SED (bottom) of the galaxy B12 in the field of view of GRB 050820A.
	 Based on the identification of [\ion{O}{ii}] $\lambda$3727 and [\ion{O}{iii}] $\lambda$5007
	 the redshift is $z=0.467$. The galaxy is not related to any of the intervening absorbers
	 seen in the afterglow spectrum.	 
	 The error spectrum is overplotted. The best fit of the SED  is shown in the bottom panel.
	 The model predicted magnitudes are superposed (squares). The gray area highlights the
	 interval that is covered by the spectrum above.
 }
  \label{fig:GRB080520A_B12}
 \end{figure}

==> tab_candidates_one_column.tex <==
\begin{table*}
\caption{Galaxy counterpart candidates of the intervening absorption line systems}
\centering
\tiny
% \begin{tabular}{l l c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c}
\begin{tabular}{l l ccc ccc cc cc}
\toprule
\multicolumn{10}{l}{\textbf{GRB 050730} (GRB: $z= 3.969$, DLA: $z= 3.56439$, sub-DLA: $z= 3.02209$, \ion{Mg}{ii} absorbers: $z=2.25313$, 1.7731)}\\ 
 Candidate  & Remark & $\theta\,(\arcsec)$ & $R$ (mag)   & $F775W$ (mag)  & $K_s$ (mag)& $3.6\,\mu\rm m$ (mag)& $5.8\,\mu\rm m$ (mag)\\                  
\midrule                                    
\textbf{A1}				&star		&12.8	&$23.46 \pm0.03	$&$23.08\pm0.01	$&$22.51\pm0.25	$\\
A2					&		&12.3	&$		$&$28.50\pm0.26	$&$		$\\						
A3					&		&10.6	&$26.53 \pm0.12	$&$26.60\pm0.09	$&$		$\\			
\textbf{A4}				&star		&7.3	&$23.88 \pm0.03	$&$23.71\pm0.02	$&$		$\\			
A5a					&		&2.5	&$27.20 \pm0.27	$&$27.98\pm0.18	$&$		$\\			
A5b\tablefootmark{a}			&		&2.1	&$		$&$28.16\pm0.19	$&$		$\\						
A5c\tablefootmark{a}			&		&2.0	&$		$&$28.43\pm0.22	$&$		$\\						
A5d					&		&1.8	&$		$&$28.84\pm0.30	$&$		$\\						
A6a					&		&1.0	&$		$&$28.64\pm0.26	$&$		$\\						
A6b					&		&0.7	&$		$&$28.37\pm0.24	$&$		$\\						
A6c					&		&0.4	&$		$&$28.11\pm0.19	$&$		$\\						
A6d					&		&1.4	&$		$&$28.64\pm0.26	$&$		$\\						
A6e					&		&0.9	&$		$&$28.64\pm0.26	$&$		$\\						
A6f					&		&1.5	&$		$&$28.29\pm0.20	$&$		$\\						
\textbf{A7}				&star		&4.2	&$23.38 \pm 0.03$&$22.84\pm0.01	$&$22.28\pm0.15	$\\
A8					&		&6.3	&$		$&$27.49\pm0.12	$&$		$\\						
A9					&		&9.8	&$		$&$27.38\pm0.12	$&$		$\\						
A10					&		&11.5	&$		$&$27.10\pm0.13	$&$		$\\						
\textbf{A11}\tablefootmark{b}		&$z\sim0.16\rm{?;}\,z<2.81$	&13.3	&$		$&$		$&$		$& & \\
\textbf{QSO}\tablefootmark{c}		&$z=3.022$	&17.5	&$20.87 \pm 0.05$&$\sim	20.58	$&$		$\\					
\textbf{Star}\tablefootmark{c}		&star		&18.3	&$18.20 \pm 0.04$&$		$&$		$\\						
% \midrule                                    
% \multicolumn{10}{l}{\textbf{GRB 050820A} (GRB: $z= 2.615$, DLA: $z= 2.3598$, \ion{Mg}{ii} absorbers: $z=1.4288$, 0.6915)}\\
%  Candidate  &  Remark &$\theta\,(\arcsec)$ &  $g$ (mag)  &  $F625W$ (mag)  &   $R$ (mag)   &  $F775W$ (mag)  &  $F850LP$ (mag)  &  $H$ (mag)  &  $K_s$ (mag) & $3.6\,\mu\rm m$ (mag)& $5.8\,\mu\rm m$ (mag)\\   
% \midrule                                    
% B1\tablefootmark{d}   			&  		& 11.8 	&$    		$&$25.18\pm0.04	$&$	    	$&$24.87\pm0.03$&$24.90\pm0.06	$&$    		$&$    		$& $23.45\pm0.30$\\
% \textbf{B2}  				& $z=0.693$ 	& 12.3 	&$ 25.41\pm0.07	$&$23.59\pm0.03	$&$23.20\pm0.03 $&$22.35\pm0.01$&$21.81\pm0.05	$&$20.81\pm0.10	$&$20.47\pm 0.05$& $20.59\pm0.05$ &$21.40\pm0.20$\\
% \textbf{B3}  				& $z=0.67^{+0.02} _{-0.07}$ & 5.2 	&$ 25.24\pm0.06 $&$23.90\pm0.04	$&$23.65\pm0.04 $&$23.01\pm0.02$&$22.57\pm0.05	$&$21.41\pm0.14	$& $21.05\pm 0.07$ &$20.94\pm0.06$ & $21.04\pm0.18$\\
% \textbf{B4} 				& star 		& 2.8 	&$ 23.39\pm0.05 $&$22.11\pm0.01	$&$21.97\pm0.03 $&$21.68\pm0.01$&$21.34\pm0.01	$&$20.94\pm0.11	$&$21.19\pm 0.07$& $21.65\pm0.10$ & $21.68\pm0.32$\\
% \textbf{B5} 				& $z=0.9\pm0.1$ & 3.7 	&$ 26.68\pm0.14 $&$26.36\pm0.09	$&$26.48\pm0.26 $&$25.58\pm0.06$&$25.36\pm0.06	$&$    		$&$		$\\
% \textbf{B6} 				& $z=1.5^{+0.2} _{-0.3}$ 	& 4.9 &$25.23\pm0.06$&$24.94\pm0.09$&$24.80\pm0.09$&$24.32\pm0.04$&$23.67\pm0.05$&$22.28\pm0.21	$&$22.20\pm0.15	$& $21.81\pm0.10$\\
% \textbf{B7}\tablefootmark{a}		& $z=2.615$ 	& 1.6 	&$ 25.75\pm0.08	$&$25.99\pm0.07	$&$25.66\pm0.10	$&$25.90\pm0.06$&$25.83\pm0.08	$&$    		$&$    		$\\
% \textbf{B8N}\tablefootmark{a} 		& \multirow{2}{*}{$z=2.615$} & 0.3&$	$&$26.16\pm0.08	$&$    		$&$25.83\pm0.08$&$26.18\pm0.06	$&$    		$&$    		$\\
% \textbf{B8S}\tablefootmark{a} 		&  		& 0.1 	&$    		$&$26.19\pm0.08	$&$		$&$25.72\pm0.07$&$25.82\pm0.05	$&$    		$&$    		$\\
% \textbf{B9}  				& $z=0.428$ 	& 3.4 	&$ 25.49\pm0.07 $&$24.94\pm0.05	$&$24.45\pm0.07	$&$24.76\pm0.03$&$24.57\pm0.04	$&$    		$&$    		$\\
% \textbf{B10}  				& star 		& 3.6 	&$ 22.11\pm0.05 $&$20.58\pm0.00	$&$20.31\pm0.03	$&$19.69\pm0.00$&$19.16\pm0.00	$&$18.60\pm0.05	$&$18.81\pm0.04	$&$19.51\pm0.03$ & $20.29\pm0.09$\\
\bottomrule                        
 \end{tabular}
\tablefoot{Observed magnitudes are given in the AB system (not corrected for Galactic extinction). VLT Vega-magnitudes
    were converted into the AB system by adding: VLT/$R$ 0.21 mag \citep{Blanton2007a}, and
    VLT/$K_s$ 1.895 mag (ESO). The selective Galactic extinctions, $E(B-V)$, is 0.051 mag.
    Impact parameters were derived from the \hst~images, if available, otherwise from $R$-band images.
    The uncertainty in the impact parameter is $0\farcs3-0\farcs4$. Spectra were extracted for boldfaced
    objects. Based on \textbf{the spectrum, the SED or the shape and colour of an object}, we report in the column
    "remark" if it is a star or at which redshift the galaxy is. The $3\sigma$ limiting magnitudes are:
    $R=27.1$, $F775W=28.6$, $K_s=22.8$, $3.5\,\mu\rm{m}=22.5$, $5.8\,\mu\rm{m}=21.5$ mag,
%     GRB 050820A: $g'=27.6$, $F625W=27.8$, $R=26.1$, $F775W=28.1$, $F850LP=28.0$, $H=23.0$, $K_s=23.0$, $3.5\,\mu\rm{m}=22.5$, $5.8\,\mu\rm{m}=22.0 mag$,
%     GRB 050908: $R=27.4$, $K_s=23.0$, and
%     GRB 070721B: $R=27.5$, $F775W=28.7$, $H=23.1$, $K_s=23.2$.
   \tablefoottext{a} {Blended object. The magnitude is only an estimate. The spectrum \textbf{can be} the
    integrated spectrum of the blended objects.}
   \tablefoottext{b}{\textbf{The object consists of at least two galaxies and is detected in all filters.
		We do not report any magnitude of the individual objects or the compound in this work. We detect
		the continuum down to 4630 \AA. If this break is caused by Ly$\alpha$ absorption, the redshift is $z=2.81$, or if
		this the redshifted 4000\,\AA~feature, the redshift is $z=0.16$.}}
   \tablefoottext{c} {The $R$-band brightness of the quasar and the star were obtained from an afterglow image
    taken on 23 February 2007 using with PSF photometry (Sect. \ref{sec:imaging}). The blended star is
    saturated in the \hst~image. The PSF was subtracted  with Tiny Tim \citep{Krist1993a} assuming
    a $FWHM$ of $5''$. While the wings of the
    star were partly removed, the residuals in the core are quite strong. The measurement of the QSO magnitude
    is only an estimate.}
%    \textbf{\tablefoottext{d}{The compound is a blend of several individual objects. We only report the brightness
%    	in the \hst~images of the brightest object.}}
}
\label{tab:candidates}
\end{table*}

\begin{sidewaystable*}
% \caption{Galaxy counterpart candidates of the intervening absorption line systems}
\centering
\tiny
% \begin{tabular}{l l c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c}
\begin{tabular}{l l ccc ccc cc cc}
\toprule
% \multicolumn{10}{l}{\textbf{GRB 050730} (GRB: $z= 3.969$, DLA: $z= 3.56439$, sub-DLA: $z= 3.02209$, \ion{Mg}{ii} absorbers: $z=2.25313$, 1.7731)}\\ 
%  Candidate  & Remark & $\theta\,(\arcsec)$ & $R$ (mag)   & $F775W$ (mag)  & $K_s$ (mag)& $3.6\,\mu\rm m$ (mag)& $5.8\,\mu\rm m$ (mag)\\                  
% \midrule                                    
% \textbf{A1}				&star		&12.8	&$23.46 \pm0.03	$&$23.08\pm0.01	$&$22.51\pm0.25	$\\
% A2					&		&12.3	&$		$&$28.50\pm0.26	$&$		$\\						
% A3					&		&10.6	&$26.53 \pm0.12	$&$26.60\pm0.09	$&$		$\\			
% \textbf{A4}				&star		&7.3	&$23.88 \pm0.03	$&$23.71\pm0.02	$&$		$\\			
% A5a					&		&2.5	&$27.20 \pm0.27	$&$27.98\pm0.18	$&$		$\\			
% A5b\tablefootmark{a}			&		&2.1	&$		$&$28.16\pm0.19	$&$		$\\						
% A5c\tablefootmark{a}			&		&2.0	&$		$&$28.43\pm0.22	$&$		$\\						
% A5d					&		&1.8	&$		$&$28.84\pm0.30	$&$		$\\						
% A6a					&		&1.0	&$		$&$28.64\pm0.26	$&$		$\\						
% A6b					&		&0.7	&$		$&$28.37\pm0.24	$&$		$\\						
% A6c					&		&0.4	&$		$&$28.11\pm0.19	$&$		$\\						
% A6d					&		&1.4	&$		$&$28.64\pm0.26	$&$		$\\						
% A6e					&		&0.9	&$		$&$28.64\pm0.26	$&$		$\\						
% A6f					&		&1.5	&$		$&$28.29\pm0.20	$&$		$\\						
% \textbf{A7}				&star		&4.2	&$23.38 \pm 0.03$&$22.84\pm0.01	$&$22.28\pm0.15	$\\
% A8					&		&6.3	&$		$&$27.49\pm0.12	$&$		$\\						
% A9					&		&9.8	&$		$&$27.38\pm0.12	$&$		$\\						
% A10					&		&11.5	&$		$&$27.10\pm0.13	$&$		$\\						
% \textbf{A11}\tablefootmark{b}		&$z\sim0.16\rm{?;}\,z<2.81$	&13.3	&$		$&$		$&$		$& & \\
% \textbf{QSO}\tablefootmark{c}		&$z=3.022$	&17.5	&$20.87 \pm 0.05$&$\sim	20.58	$&$		$\\					
% \textbf{Star}\tablefootmark{c}		&star		&18.3	&$18.20 \pm 0.04$&$		$&$		$\\						
% \midrule                                    
\multicolumn{10}{l}{\textbf{GRB 050820A} (GRB: $z= 2.615$, DLA: $z= 2.3598$, \ion{Mg}{ii} absorbers: $z=1.4288$, 0.6915)}\\
 Candidate  &  Remark &$\theta\,(\arcsec)$ &  $g$ (mag)  &  $F625W$ (mag)  &   $R$ (mag)   &  $F775W$ (mag)  &  $F850LP$ (mag)  &  $H$ (mag)  &  $K_s$ (mag) & $3.6\,\mu\rm m$ (mag)& $5.8\,\mu\rm m$ (mag)\\   
\midrule                                    
B1\tablefootmark{d}   			&  		& 11.8 	&$    		$&$25.18\pm0.04	$&$	    	$&$24.87\pm0.03$&$24.90\pm0.06	$&$    		$&$    		$& $23.45\pm0.30$\\
\textbf{B2}  				& $z=0.693$ 	& 12.3 	&$ 25.41\pm0.07	$&$23.59\pm0.03	$&$23.20\pm0.03 $&$22.35\pm0.01$&$21.81\pm0.05	$&$20.81\pm0.10	$&$20.47\pm 0.05$& $20.59\pm0.05$ &$21.40\pm0.20$\\
\textbf{B3}  				& $z=0.67^{+0.02} _{-0.07}$ & 5.2 	&$ 25.24\pm0.06 $&$23.90\pm0.04	$&$23.65\pm0.04 $&$23.01\pm0.02$&$22.57\pm0.05	$&$21.41\pm0.14	$& $21.05\pm 0.07$ &$20.94\pm0.06$ & $21.04\pm0.18$\\
\textbf{B4} 				& star 		& 2.8 	&$ 23.39\pm0.05 $&$22.11\pm0.01	$&$21.97\pm0.03 $&$21.68\pm0.01$&$21.34\pm0.01	$&$20.94\pm0.11	$&$21.19\pm 0.07$& $21.65\pm0.10$ & $21.68\pm0.32$\\
\textbf{B5} 				& $z=0.9\pm0.1$ & 3.7 	&$ 26.68\pm0.14 $&$26.36\pm0.09	$&$26.48\pm0.26 $&$25.58\pm0.06$&$25.36\pm0.06	$&$    		$&$		$\\
\textbf{B6} 				& $z=1.5^{+0.2} _{-0.3}$ 	& 4.9 &$25.23\pm0.06$&$24.94\pm0.09$&$24.80\pm0.09$&$24.32\pm0.04$&$23.67\pm0.05$&$22.28\pm0.21	$&$22.20\pm0.15	$& $21.81\pm0.10$\\
\textbf{B7}\tablefootmark{a}		& $z=2.615$ 	& 1.6 	&$ 25.75\pm0.08	$&$25.99\pm0.07	$&$25.66\pm0.10	$&$25.90\pm0.06$&$25.83\pm0.08	$&$    		$&$    		$\\
\textbf{B8N}\tablefootmark{a} 		& \multirow{2}{*}{$z=2.615$} & 0.3&$	$&$26.16\pm0.08	$&$    		$&$25.83\pm0.08$&$26.18\pm0.06	$&$    		$&$    		$\\
\textbf{B8S}\tablefootmark{a} 		&  		& 0.1 	&$    		$&$26.19\pm0.08	$&$		$&$25.72\pm0.07$&$25.82\pm0.05	$&$    		$&$    		$\\
\textbf{B9}  				& $z=0.428$ 	& 3.4 	&$ 25.49\pm0.07 $&$24.94\pm0.05	$&$24.45\pm0.07	$&$24.76\pm0.03$&$24.57\pm0.04	$&$    		$&$    		$\\
\textbf{B10}  				& star 		& 3.6 	&$ 22.11\pm0.05 $&$20.58\pm0.00	$&$20.31\pm0.03	$&$19.69\pm0.00$&$19.16\pm0.00	$&$18.60\pm0.05	$&$18.81\pm0.04	$&$19.51\pm0.03$ & $20.29\pm0.09$\\
\bottomrule                        
 \end{tabular}
\tablefoot{Observed magnitudes are given in the AB system (not corrected for Galactic extinction). VLT and Magellan Vega-magnitudes
    were converted into the AB system by adding: VLT/$R$ 0.21 mag \citep{Blanton2007a},
    VLT/$K_s$ 1.895 mag (ESO), and Magellan/$H$ 1.34 mag. The selective Galactic extinctions, $E(B-V)$. is 0.044 mag.
    Impact parameters were derived from the \hst~images, if available, otherwise from $R$-band images.
    The uncertainty in the impact parameter is $0\farcs3-0\farcs4$. Spectra were extracted for boldfaced
    objects. Based on \textbf{the spectrum, the SED or the shape and colour of an object}, we report in the column
    "remark" if it is a star or at which redshift the galaxy is. The $3\sigma$ limiting magnitudes are:
%     GRB 050730: $R=27.1$, $F775W=28.6$, $K_s=22.8$, $3.5\,\mu\rm{m}=22.5$, $5.8\,\mu\rm{m}=21.5$ mag,
%     GRB 050820A:
    $g'=27.6$, $F625W=27.8$, $R=26.1$, $F775W=28.1$, $F850LP=28.0$, $H=23.0$, $K_s=23.0$, $3.5\,\mu\rm{m}=22.5$, $5.8\,\mu\rm{m}=22.0 mag$,
%     GRB 050908: $R=27.4$, $K_s=23.0$, and
%     GRB 070721B: $R=27.5$, $F775W=28.7$, $H=23.1$, $K_s=23.2$.
   \tablefoottext{a} {Blended object. The magnitude is only an estimate. The spectrum \textbf{can be} the
    integrated spectrum of the blended objects.}
%    \tablefoottext{b}{\textbf{The object consists of at least two galaxies and is detected in all filters.
% 		We do not report any magnitude of the individual objects or the compound in this work. We detect
% 		the continuum down to 4630 \AA. If this break is caused by Ly$\alpha$ absorption, the redshift is $z=2.81$, or if
% 		this the redshifted 4000\,\AA~feature, the redshift is $z=0.16$.}}
%    \tablefoottext{c} {The $R$-band brightness of the quasar and the star were obtained from an afterglow image
%     taken on 23 February 2007 using with PSF photometry (Sect. \ref{sec:imaging}). The blended star is
%     saturated in the \hst~image. The PSF was subtracted  with Tiny Tim \citep{Krist1993a} assuming
%     a $FWHM$ of $5''$. While the wings of the
%     star were partly removed, the residuals in the core are quite strong. The measurement of the QSO magnitude
%     is only an estimate.}
   \textbf{\tablefoottext{d}{The compound is a blend of several individual objects. We only report the brightness
   	in the \hst~images of the brightest object.}}
}
\hfill\center{Tab. \ref{tab:candidates} --- continued}
\end{sidewaystable*}

\begin{table*}
\centering
\tiny
% \begin{tabular}{l l c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c}
\begin{tabular}{l l ccc ccc}
\toprule
% \multicolumn{10}{l}{\textbf{GRB 050730} (GRB: $z= 3.969$, sub-DLA: $z= 3.02209$, DLA: $z= 3.56439$, weak \ion{Mg}{ii} absorber: $2.25313$, strong \ion{Mg}{ii} absorber: $1.7731$)asdfasdf}\\ 
\multicolumn{8}{l}{\textbf{GRB 050908} (DLA: $z= 3.3467$, DLA: $z= 2.6208$, \ion{Mg}{ii} absorber: $z=1.5481$)}\\
 Candidate   		& Remark & $\theta\,(\arcsec)$ & $R$ (mag)  & $K_s$ (mag) & $3.6\,\mu\rm m$ (mag)& $5.8\,\mu\rm m$ (mag)&\\
\midrule                        
\textbf{C1 } 		& $z\approx2.71$& 12.6 &$ 27.10 \pm 0.20 $& &\\            
C2   			& 		& 11.5 &$ 24.96 \pm 0.04 $& &$23.25\pm0.19$\\
C3   			& 		& 6.6 &$ 25.97 \pm 0.09 $& &\\            
C4\tablefootmark{a} 	& 	 	& 12.4 &$ 26.17 \pm 0.09 $& &\\            
C5\tablefootmark{a,b}	&  		& 3.7 &$ 25.05 \pm 0.04 $ && $23.65\pm0.23$&$22.44\pm0.44$\\
C6\tablefootmark{a,b} 	&  		& 2.8 &$ 25.39 \pm 0.05 $& &\\            
C7\tablefootmark{b}	& 		& 1.1 &$ 26.98 \pm 0.18 $& &\\            
C8			&  		& 5.5 &$ 26.59 \pm 0.21 $& &\\            
C9		   	& 		& 2.5 &$ 25.96 \pm 0.12 $& &$\sim25.0\pm0.5$&\\            
\midrule                        
\multicolumn{8}{l}{\textbf{GRB 070721B} (GRB: $z= 3.6298$, DLA: $z= 3.0939$)}\\                       
 Candidate   & Remark & $\theta\,(\arcsec)$ & $R$ (mag)  & $F775W$ (mag)  & $H$ (mag)  & $K_s$ (mag)\\   
\midrule                        
D1   				&  					& 12.8 &$    $&$ 27.40 \pm 0.12 $&$    $&$    $\\
\textbf{D2a}\tablefootmark{a} 	& \multirow{2}{*}{$z\approx2.64$} 	& 3.0 &$    $&$ 27.34 \pm 0.12 $&$    $&$    $\\
\textbf{D2b}\tablefootmark{a} 	& 				 	& 2.8 &$    $&$ 28.23 \pm 0.22 $&$    $&$    $\\
\textbf{D3 }  			& $z=3.096$			 	& 1.0 &$ 24.48 \pm 0.02 $&$ 24.41 \pm 0.02 $&$ 23.40 \pm 0.07 $&$ 23.56 \pm 0.23 $\\
\textbf{D4 } 			& $z=3.631$ 				& 0.1 &$    $&$ 27.31 \pm 0.15 $&$    $&$    $\\
D5  				&  					& 6.9 &$ 26.82 \pm 0.18 $&$ 26.44 \pm 0.10 $&$    $&$    $\\
\textbf{D6a}\tablefootmark{a} 	& \multirow{2}{*}{$z\approx2.64$} 	& 11.7 &$    $&$ 25.05 \pm 0.04 $&$    $&$    $\\
\textbf{D6b}\tablefootmark{a} 	&  					& 12.2 &$    $&$ 26.90 \pm 0.09 $&$    $&$    $\\
\textbf{D7}  			& $z=3.615$ 				& 20.7 &$ 23.77 \pm 0.01 $&$ 23.74 \pm 0.03 $&$ 24.02 \pm 0.11 $&$ 23.20 \pm 0.17 $\\
\bottomrule
\end{tabular}
\tablefoot{The selective Galactic extinctions, $E(B-V)$, are 0.025 and 0.031 mag for GRBs 050908 and 070721B, respectively.
    Spectra were extracted for boldfaced objects. Based on the spectrum or the SED of an object, we show in the column
    "remark" if it is a star or at which redshift the galaxy is. The $3\sigma$ limiting magnitudes are:
    GRB 050908: $R=27.4$, $K_s=23.0$, $3.6\,\mu\rm m= 22.8$, $5.8\,\mu\rm m= 22.3$ mag and
    GRB 070721B: $R=27.5$, $F775W=28.7$, $H=23.1$, $K_s=23.2$ mag.
    \tablefoottext{a} {Blended object. The magnitude is only an estimate. The spectrum is the
    integrated spectrum of the blended objects.}
    \tablefoottext{b} {We do not attempt photometry on objects which are strongly blended in
    the \spitzer~data in this work, with the exception of objects C5, C6, and C7, which are sufficiently closely
    blended that we report the (summed) photometry of all three objects as a group.}
}
\hfill\center{Tab. \ref{tab:candidates} --- continued}
\end{table*}
% 
% \begin{table*}
% \caption{Galaxy counterpart candidates of the intervening absorption line systems}
% \centering
% \tiny
% % \begin{tabular}{l l c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c@{\hspace{2mm}}c}
% \begin{tabular}{l l ccc ccc cc}
% \toprule
%            
% \multicolumn{10}{l}{\textbf{GRB 050820A} (GRB: $z= 2.615$, DLA: $z= 2.3598$, weak \ion{Mg}{ii} absorber: $z=1.6204$, strong \ion{Mg}{ii} absorbers: $z=1.4288$ and 0.6915)}\\
%  Candidate  &  Remark &$\theta\,(\arcsec)$ &  $g$ (mag)  &  $F625W$ (mag)  &   $R$ (mag)   &  $F775W$ (mag)  &  $F850LP$ (mag)  &  $H$ (mag)  &  $K_s$ (mag)\\   
% \midrule                                    
% B1\tablefootmark{b}   			&  		& 11.8 	&$    		$&$25.18\pm0.04	$&$	    	$&$24.87\pm0.03$&$24.90\pm0.06	$&$    		$&$    		$\\
% \textbf{B2}  				& $z=0.693$ 	& 12.3 	&$ 25.41\pm0.07	$&$23.59\pm0.03	$&$23.20\pm0.03 $&$22.35\pm0.01$&$21.81\pm0.05	$&$20.81\pm0.10	$&$20.47\pm 0.05$\\
% \textbf{B3}  				& $z=0.67^{+0.02} _{-0.07}$ & 5.2 	&$ 25.24\pm0.06 $&$23.90\pm0.04	$&$23.65\pm0.04 $&$23.01\pm0.02$&$22.57\pm0.05	$&$21.41\pm0.14	$&$21.05\pm 0.07$\\
% \textbf{B4} 				& star 		& 2.8 	&$ 23.39\pm0.05 $&$22.11\pm0.01	$&$21.97\pm0.03 $&$21.68\pm0.01$&$21.34\pm0.01	$&$20.94\pm0.11	$&$21.19\pm 0.07$\\
% \textbf{B5} 				& $z=0.9\pm0.1$ & 3.7 	&$ 26.68\pm0.14 $&$26.36\pm0.09	$&$26.48\pm0.26 $&$25.58\pm0.06$&$25.36\pm0.06	$&$    		$&$		$\\
% \textbf{B6} 				& $z=1.5^{+0.2} _{-0.3}$ 	& 4.9 &$25.23\pm0.06$&$24.94\pm0.09$&$24.80\pm0.09$&$24.32\pm0.04$&$23.67\pm0.05$&$22.28\pm0.21	$&$22.20\pm0.15	$\\
% \textbf{B7}\tablefootmark{b}		& $z=2.615$ 	& 1.6 	&$ 25.75\pm0.08	$&$25.99\pm0.07	$&$25.66\pm0.10	$&$25.90\pm0.06$&$25.83\pm0.08	$&$    		$&$    		$\\
% \textbf{B8N}\tablefootmark{b} 		& \multirow{2}{*}{$z=2.615$} & 0.3&$	$&$26.16\pm0.08	$&$    		$&$25.83\pm0.08$&$26.18\pm0.06	$&$    		$&$    		$\\
% \textbf{B8S}\tablefootmark{b} 		&  		& 0.1 	&$    		$&$26.19\pm0.08	$&$		$&$25.72\pm0.07$&$25.82\pm0.05	$&$    		$&$    		$\\
% \textbf{B9}  				& $z=0.428$ 	& 3.4 	&$ 25.49\pm0.07 $&$24.94\pm0.05	$&$24.45\pm0.07	$&$24.76\pm0.03$&$24.57\pm0.04	$&$    		$&$    		$\\
% \textbf{B10}  				& star 		& 3.6 	&$ 22.11\pm0.05 $&$20.58\pm0.00	$&$20.31\pm0.03	$&$19.69\pm0.00$&$19.16\pm0.00	$&$18.60\pm0.05	$&$18.81\pm0.04	$\\
% \midrule    
% \multicolumn{10}{l}{\textbf{GRB 050908} (DLA: $z= 3.3467$, DLA: $z= 2.6208$, \ion{Mg}{ii} absorber: $z=1.5481$)}\\
%  Candidate   & Remark & $\theta\,(\arcsec)$ & $R$ (mag)  & $K_s$ (mag)\\          
% \midrule                        
% \textbf{C1 } 		& $z\approx2.71$& 12.6 &$ 27.10 \pm 0.20 $\\            
% C2   			& 		& 11.5 &$ 24.96 \pm 0.04 $\\            
% C3   			&  		& 6.6 &$ 25.97 \pm 0.09 $\\            
% C4\tablefootmark{b} 	&  		& 12.4 &$ 26.17 \pm 0.09 $\\            
% C5\tablefootmark{b} 	&  		& 3.7 &$ 25.05 \pm 0.04 $\\            
% C6\tablefootmark{b} 	&  		& 2.8 &$ 25.39 \pm 0.05 $\\            
% C7	   		& 		& 1.1 &$ 26.98 \pm 0.18 $\\            
% C8		   	&  		& 5.5 &$ 26.59 \pm 0.21 $\\            
% C9		   	& 		& 2.5 &$ 25.96 \pm 0.12 $\\            
% \midrule                        
% \multicolumn{10}{l}{\textbf{GRB 070721B} (GRB: $z= 3.6298$, DLA: $z= 3.0939$)}\\                       
%  Candidate   & Remark & $\theta\,(\arcsec)$ & $R$ (mag)  & $F775W$ (mag)  & $H$ (mag)  & $K_s$ (mag)\\   
% \midrule                        
% D1   				&  					& 12.8 &$    $&$ 27.40 \pm 0.12 $&$    $&$    $\\
% \textbf{D2a}\tablefootmark{b} 	& \multirow{2}{*}{$z\approx2.64$} 	& 3.0 &$    $&$ 27.34 \pm 0.12 $&$    $&$    $\\
% \textbf{D2b}\tablefootmark{b} 	& 				 	& 2.8 &$    $&$ 28.23 \pm 0.22 $&$    $&$    $\\
% \textbf{D3 }  			& $z=3.096$			 	& 1.0 &$ 24.48 \pm 0.02 $&$ 24.41 \pm 0.02 $&$ 23.40 \pm 0.07 $&$ 23.56 \pm 0.23 $\\
% \textbf{D4 } 			& $z=3.631$ 				& 0.1 &$    $&$ 27.31 \pm 0.15 $&$    $&$    $\\
% D5  				&  					& 6.9 &$ 26.82 \pm 0.18 $&$ 26.44 \pm 0.10 $&$    $&$    $\\
% \textbf{D6a}\tablefootmark{b} 	& \multirow{2}{*}{$z\approx2.64$} 	& 11.7 &$    $&$ 25.05 \pm 0.04 $&$    $&$    $\\
% \textbf{D6b}\tablefootmark{b} 	&  					& 12.2 &$    $&$ 26.90 \pm 0.09 $&$    $&$    $\\
% % D7   &  & 15.17 &$ 25.89 \pm 0.08 $&$ 27.47 \pm 0.13 $&$    $&$    $\\
% \textbf{D7}  			& $z=3.615$ 				& 20.7 &$ 23.77 \pm 0.01 $&$ 23.74 \pm 0.03 $&$ 24.02 \pm 0.11 $&$ 23.20 \pm 0.17 $\\
% \bottomrule                        
%  \end{tabular}
% \hfill\center{Tab. \ref{tab:candidates} --- continued}
% \end{table*}

